Revisiting Embeddings for Graph Neural Networks

Current graph representation learning techniques use Graph Neural Networks (GNNs) to extract features from dataset embeddings. In this work, we examine the quality of these embeddings and assess how changing them can affect the accuracy of GNNs. We explore different embedding extraction techniques for both images and texts; and find that the performance of different GNN architectures is dependent on the embedding style used. We see a prevalence of bag of words (BoW) embeddings and text classification tasks in available graph datasets. Given the impact embeddings has on GNN performance. this leads to a phenomenon that GNNs being optimised for BoW vectors.

==> old-sections/background.tex <==
\section{Background}
\label{sec:background}
\input{tables/dataset-overview}

We compare our new method (GraNet) against some standard Graph Neural Networks to demonstrate the improvements that GraNet makes in classifying datasets.

\citet{Kipf:2017tc} introduce GCN (Graph Convolutional Networks) -- a method of applying convolutional layers from CNNs to graph neural networks. It focuses on spectral filters applied to the whole graph structure rather than at the node level.

\citet{Hamilton:2017tp} introduce the GraphSAGE model which builds on prior work from GCN focusing on individual node representations. This gives rise to the iterative message passing process on the node level. Though simpler than newer models we find that this approach, when given the right embedding style, can outperform some recently published GNNs.

\citet{Velickovic:2018we} introduce the idea of graph attention which alters how a node aggregates its neighbours representation. This adds an additional attention mechanism to discern which aspects of the node representations in a nodes neighbourhood are important at a given layer. 

\citet{Brody2021GATv2} provide a more attentive version based on the graph attention system introduced in \citet{Velickovic:2018we}. We base the graph attention mechanism used in our GraNet models on this improved version of graph attention. We provide both versions of graph attention in our results to compare to our new approach.

\subsection{Notations}
\textbf{Graph Data}
\label{sec:background:preliminary}
Let $\gG(\sV, \mathcal{E}, \mX)$ denote a graph where $\sV = \{\vv_1, \vv_2, ..., \vv_n\}$ is the set of nodes and $N=|\sV|$ is the number of nodes in the graph, $\mathcal{E}$ is the set of edges between nodes in $\sV$ such that $\ve_{i,j} \in \mathcal{E}$ denotes a directed connection from node $\vv_i$ to node $\vv_j$, $\ve_{i,j}$ may itself be a feature vector.
We say each node $\vv_i$ has a neighbourhood $\sN_i$ such that $\vv_j \in \sN_i \iff \ve_{j,i} \in \mathcal{E}$ and we say that $\vv_j$ is a neighbour node to $\vv_i$. Where $\mX$ is the raw data matrix where $\mX_{:, i} = \vx_i$ where $\vx_i$ is the feature vector for node $\vv_i$.

\textbf{Embeddings} 
\label{eq:embedding}
There normally exists a transformation function, $f_e$, to project the raw data to a more compact feature $\mX_e$ space such that $\mX_e = f_e(\mX)$ 

For instance, we can transform a set of images ($\mX \in \sR^{N \times C \times H \times W}$, where $C$, $H$ and $W$ are the number of channels, width and height of an image) to 1D features ($\mX_e \in \sR^{N \times F}$, where $F$ denotes the feature dimension). In this case, we have an embedding function $f_e: \sR^{N \times C \times H \times W} \rightarrow \mathbb{R}^{N \times F}$ for the dimensional reduction.

This paper puts a special focus on the design of $f_e$, and reveals later how the design choice of $f_e$ can influence the performance of GNN models without making any changes to the underlying data $\gG(\sV, \mathcal{E}, \mX)$. An overview of popular datasets, and the embeddings that they use, is presented in \Cref{tab:dataset-overview}. We see that the popular graph datasets \citep{zeng2019graphsaint,Kipf:2017tc,shchur2018pitfalls,Hamilton:2017tp} focus heavily on Bag of Words (BoW) and word vectors. This implies that current GNNs are being tested on and designed for a very narrow class of embedding styles.
A more detailed discussion is available in \Cref{sec:app:dataset-overview}.

\textbf{Graph Neural Networks} Current GNNs can be thought of as \emph{message passing} layers, the $l$-th layer can be represented as
%\vspace{-10pt}

\begin{equation}
\label{eq:messagepassing}
\vh_i^{l} = \gamma_{\vtheta_\gamma} \left(\vh^{l-1}_i,
        \psi_{j \in \sN(i)} \left( \phi_{\vtheta_\phi}
        \left(\vh^{l-1}_i, \vh^{l-1}_j,\ve_{j,i}\right) \right) \right)
\end{equation}
% \vspace{-10pt}

where $\psi$ is a differentiable aggregation function and $\gamma_{\vtheta_\gamma}$ and $\phi_{\vtheta_\phi}$ represent differentiable functions with trainable parameters $\vtheta_\gamma$ and ${\vtheta_\phi}$ respectively. $\vh^l_i$ is the node representation of $v_i$ at layer $l$, with $\vh^0_i = f_e(\vx_i)$.

We focus on the improved graph attention mechanism \citep{Brody2021GATv2} when looking at potential GNNs for GraNet. Using this new notation we can formulate it as such

\begin{equation}
    \label{eq:GATv2}
    \alpha_{ij} = \frac{exp(\bm{a}^T\mbox{LeakyReLU}(\bm{\theta}[\bm{h}_i||\bm{h}_j]))}{\sum_{k \in \sN_i} exp(\bm{a}^T\mbox{LeakyReLU}(\bm{\theta}[\bm{h}_i||\bm{h}_j]))}
\end{equation}

where $\bm{a}$ is a learnable parameter representing the attention of the network. Further discussion of graph attention and why this is useful in GraNet is available in \Cref{sec:app:models}.

\textbf{Pre-trained models} are specific neural network architecturwa that have been trained on a dataset $\mathcal{D}$ for a specific task, this could be ImageNet classification \citep{deng2009imagenet} for vision networks \citep{he2016deep} or the entire English Wikipedia for language models \citep{liu2019roberta}. These networks therefore have \textit{pre-trained} weights $\bm{\theta}$ that can be loaded into the model for further training or evaluation.

We denote these pre-trained models as $f_{\vtheta}$ that is parameterised by weights $\bm{\theta}$. We say that a pre-trained model has a set of functions $\{f^1_{\vtheta_1}, f^2_{\vtheta_2}, ..., f^M_{\vtheta_M} \}$ for an $M$-layer model, where $f^i_{\vtheta_i} : \sR^F \rightarrow \sR^{F^\prime}$ and $f^{i+1}_{\vtheta_{i+1}} : \sR^{F^\prime} \rightarrow \sR^{F^{\prime\prime}}$ and $F$ is the feature dimension. 
A pass through a single layer, $l$, of a network would be $f^l_{\vtheta_l}(\vx)$, shorthand for $f^l(\vx; \vtheta_l)$.
If we concatenate these layers to form a full pass through the network, we obviously have $f_{\vtheta}(\vx) = f^M_{\vtheta_M}(...f^2_{\vtheta_2}(f^1_{\vtheta_1}(\vx)))$

\textbf{Fine-tuning} is therefore adapting $\vtheta$ to a new dataset $\mathcal{D}^\prime$ which is related to $\mathcal{G}(\sV, \mathcal{E}, \mX)$ as illustrated in \Cref{sec:background:preliminary}. 
In a more standard setup, the target dataset we fine-tune to has the same underlying data-structure as the pre-training dataset, for instance, they might both be images, but the target dataset is a different type of classification. This may involve adding, removing or altering specific layers within the model or simply retraining the model with different labels on $\mathcal{D}$.

If the architecture of a pre-trained model is altered then a new weight matrix $\vtheta^\prime$ must be created from $\vtheta$ by adding, removing or reshaping weights.

\textbf{Freezing} layers is the process whereby a selection of weights $\vtheta_f \subset \vtheta$ do not have gradients and thus do not change during back-propagation.

These ideas allow us to alter these pre-trained models to use information about the graph connections whilst utilising their pre-trained weight $\vtheta$. 

\textbf{Blending and Fine-tuning} models is therefore the process of using existing models, $f_{\vtheta_f}$ and $g_{\vtheta_g}$, with defined set of layers, $\{f^1_{\vtheta_{f1}}, f^2_{\vtheta_{f2}}, ..., f^N_{\vtheta_{fN}} \}$ and $\{g^1_{\vtheta_{g1}}, g^2_{\vtheta_{g2}}, ..., g^M_{\vtheta_{gM}} \}$, and creating a new model, $h_{\vtheta_{f,g}}$, such that $h^i_{\vtheta_{f,g}} = f^j_{\vtheta_f} \circ g^k_{\vtheta_g}$. We can use pre-trained weights $\vtheta_f$ or $\vtheta_g$ and/or freeze either model, and where one of these models is a GNN we say this is fine-tuning on a graph dataset.

\textbf{Unconnected models} are models that, unlike GNNs, do not use any information about graph connections within a dataset. These are trained on datasets that are not graph-connected where each datapoint is consider isolated. We focus on complex unconnected models with multiple layers, such as vision networks, which we call \textit{large models}. Due to training cost we use \textit{pre-trained large models}.

==> old-sections/conclusion.tex <==
\section{Conclusion}
In this paper, we reveal that GNN model designs are overfitting to certain embeddings styles (\textit{e.g.} BoW and word vectors). To demonstrate this we introduced three new datasets each with a range of embedding styles to be used as a more comprehensive benchmark of GNN performance. 

We demonstrated that embedding style influences the performance of GNNs regardless of the underlying dataset. Equally, the quality of the embedding, measured by how well an unconnected baseline model performs, is a greater indicator of GNN accuracy than the GNN architecture chosen. \emph{We therefore stress the importance of creating high quality embeddings} and \emph{choosing the best GNN architecture based on the style of embedding} created rather than using (or trying to improve) the same GNN model for every task.

We then introduced a new approach named GraNet. \emph{This approach allows for any large pre-trained model to be fine-tuned to a graph-connected dataset} by altering the standard message passing function. In this way we exploit graph structure information to enhance the pre-trained model performance on graph-connected datasets. We have demonstrated that \emph{GraNet outperforms both unconnected pre-trained models and GNNs} on a range of datasets.

There is an increasing trend towards large pre-trained models and graph-connected datasets. 
Our work demonstrates potential pitfalls in the way GNN architectures are currently evaluated and proposes a new technique to fully exploit the benefits of pre-trained models within a GNN.
\newpage

==> old-sections/datasets.tex <==
\section{Our Datasets}
\label{sec:app:datasets}
\input{tables/dataset-flickr}

In this paper we look at the Flickr \citep{Hamilton:2017tp} and Amazon \citep{Hamilton:2017tp, shchur2018pitfalls} datasets (specifically looking at the Electronics and Instruments subsection of Amazon). An overview of the provided datasets and embeddings is present in \Cref{tab:flickr-dataset}.

As demonstrated in \Cref{sec:related} the process of building a graph dataset is currently signified by choosing an embedding function $f_e$ to apply to the underlying dataset $\bm{X}$. We provide three cases of the underlying dataset $\bm{X}$ and provide a selection of embeddings from sensible embedding functions. We also provide a \textit{raw} graph-connected image dataset, by which we mean the underlying image dataset $\bm{X}$ is not reduced to a matrix of 1D feature vectors but remains a multi-dimensional tensor of multi-dimensional image tensors.

As discussed in \Cref{sec:related}, versions of these datasets \citep{zeng2019graphsaint,shchur2018pitfalls}
utilize classical word embeddings. We propose using large pre-trained models as embedding functions as these can extract richer features ($\displaystyle \mX_e$) that may better represent the underlying data ($\bm{X}$) of the dataset. 

We will host our datasets in a website and make both these baselines and datsets accessible to the community (website link will be added after acceptance).

\subsection{Flickr\_v2}
The prior Flickr \citep{zeng2019graphsaint}
dataset does not contain the raw image data nor the flickr identifiers only the embeddings created in \textit{McAuley et al.} \cite{McAuley2012image} but
SNAP provides an adjacency matrix and flickr identifiers. We follow how \textit{Zeng et al.} \cite{zeng2019graphsaint} generated their dataset by downloading all the images still available, but we are unable to match the exact images they sourced or the labels. This does mean we cannot directly compare results but we find that the benchmark results we have achieved are similar.

As shown in \Cref{tab:dataset-overview} Flickr uses BoW but as discussed in \Cref{sec:setup:flickr} we deem this inappropriate for the image dataset. A potential solution would be to process the images, as discussed, to create text descriptions that can be converted into BoW embeddings. However, this would either require a human, and thus the benefits of using a neural network (such as time efficiency of classification) is lost, or a neural network. In the case of a neural network we claim that the provided networks for image classification would perform better. This is an area for further investigation especially as we found BoW works better in the case of Amazon Instruments.

As the dataset is created from four separate image classification challenges \citep{Everingham15, nus-wide-civr09, huiskes08} the existing labels and tags for these datasets are not well aligned. We therefore only select the NUS-Wide \citep{nus-wide-civr09} subsection. To create labels for our dataset we use GloVe to generate vector representations of the NUS-Wide tags and find the closest vector representation of 7 hand-picked labels.

The hand-picked labels: [``People", ``Buildings", ``Places", ``Plants", ``Animals", ``Vehicles", ``Scenery"]

This new dataset we call Flickr\_v2. 

\subsection{AmazonElectronics and AmazonInstruments}
We use the review text as our raw input features, this means a number of Amazon items are unsuitable as they do not have any reviews. The connections between nodes are based on Amazons three similarity metric ``Co-viewed", ``Co-bought" and ``Similar Items". We only consider direct connections between nodes in a specific Amazon category (in our case Electronics and instruments) making sure removing any nodes that are not directly connected to another node.

Amazon products do not belong to a single category and therefore a products categories are closer to tags than labels. Thus, similar to Flickr\_v2, we use GloVe word vectors to label our dataset based on the set of categories that each product belongs to against a hand-picked selection of categories.

Hand-picked labels for Electronics: [``Camera Photo and Lighting", ``Audio and Video", ``Bags, Cases and Covers", ``Batteries and Chargers", ``Peripherals, Keyboards and Mice", ``Storage and Networking"]

Hand-picked labels for Instruments: [``Electric Guitar", ``Acoustic Guitar", ``Percussion", ``Live Sound \& Stage", ``Studio Recording Equipment", ``Microphones \& Cable", ``Amplifiers \& Effects"]

These new datasets we call AmazonElectronics and AmazonInstruments.

The statistics for these datasets is available in \Cref{tab:flickr-dataset}

==> old-sections/definitions.tex <==
\section{Definitions}
\label{sec:app:definition}

\textbf{Pre-trained models} are models where a specific neural network architecture exists that have been trained on a dataset $\mathcal{D}$ for a specific task, this could be ImageNet classification \citep{deng2009imagenet} for vision networks \cite{he2016deep} or the entire English Wikipedia for language models \cite{liu2019roberta}. These networks therefore have \textit{pre-trained} weights $\bm{\theta}$ that can be loaded into the model for further training or evaluation.

We denote these pre-trained models as $f_{\bm{\theta}}$ that is parameterised by weights $\bm{\theta}$. We say that a pre-trained model has a set of functions $\{f^1_{\bm{\theta}_1}, f^2_{\bm{\theta}_2}, ..., f^M_{\bm{\theta}_M} \}$ for an $M$-layer model, where $f^i_{\bm{\theta}_i} : \mathbb{R}^F \rightarrow \mathbb{R}^{F^\prime}$ and $f^{i+1}_{\bm{\theta}_{i+1}} : \mathbb{R}^{F^\prime} \rightarrow \mathbb{R}^{F^{\prime\prime}}$ and $F$ is the feature dimension. 
If we concatenate these layers, we obviously have $f_{\bm{\theta}}(x) = f^M_{\bm{\theta}_M}(...f^2_{\bm{\theta}_2}(f^1_{\bm{\theta}_1}(x)))$

\textbf{Fine-tuning} is therefore adapting $\bm{\theta}$ to a new dataset $\mathcal{D}^\prime$ which is related to $\mathcal{G}(\mathcal{V}, \mathcal{E}, \bm{X})$ as illustrated in \Cref{sec:related:preliminary}. 

In a more standard setup, the target dataset we fine-tune to has the same underlying data-structure as the pre-training dataset, for instance, they might both be images, but the target dataset is a different type of classification. This may involve adding, removing or altering specific layers within the model or simply retraining the model with different labels on $\mathcal{D}$.

If the architecture of a pre-trained model is altered then a new weight matrix $\bm{\theta}^\prime$ must be created from $\bm{\theta}$ by adding, removing or reshaping weights.

\textbf{Freezing} layers is the process whereby a selection of weights $\bm{\theta}_f \subset \bm{\theta}$ do not have gradients and thus do not change during back-propagation.

These ideas allow us to alter these pre-trained models to use information about the graph connections whilst utilising their pre-trained weight $\bm{\theta}$. 

\textbf{Blending and Fine-tuning} models is therefore the process of using existing models, $f_{\bm{\theta}_f}$ and $g_{\bm{\theta}_g}$, with defined set of layers, $\{f^1_{\bm{\theta}_{f1}}, f^2_{\bm{\theta}_{f2}}, ..., f^N_{\bm{\theta}_{fN}} \}$ and $\{g^1_{\bm{\theta}_{g1}}, g^2_{\bm{\theta}_{g2}}, ..., g^M_{\bm{\theta}_{gM}} \}$, and creating a new model, $h_{\bm{\theta}_{f,g}}$, such that $h^i_{\bm{\theta}_{f,g}} = f^j_{\bm{\theta}_f} \circ g^k_{\bm{\theta}_g}$. We can use pre-trained weights $\bm{\theta}_f$ or $\bm{\theta}_g$ and/or freeze either model, and where one of these models is a GNN we say this is fine-tuning on a graph dataset.

==> old-sections/discussion.tex <==
\section{Discussion}

\textbf{Discuss smoothness of the embeddings}

==> old-sections/ethics.tex <==
\section{Ethics Statement}

With all computer based research there is the issue of carbon footprint. Each train, validation and test run of a model requires electricity which is currently largely sourced from fossil fuels. This training cost carbon footprint is present in this picture, and attempts to keep this low by running short test on new iterations rather than long runs which could waste GPU time and energy.

==> old-sections/evaluation.tex <==
\section{Evaluation}
\label{sec:eval}

% For convenience we have split each dataset into two tables: the first comparing current GNN models across the different embeddings and against pre-trained models designed for the specific task, the second comparing the new transfer learning approaches against the best performing GNN and the non-graphly-connected pre-trained, fine-tuned model.
% \vspace{-10pt}
\subsection{Re-evaluating Embeddings}

\textbf{Language Tasks}
% \label{sec:eval:language}
\Cref{tab:amazon} demonstrates that the particular embedding function used determines which GNN model performs best on the dataset.
% the style of the embeddings has a very large impact on which type of GNN architecture should be used. 
For instance, GAT2 has the best performance if the data is embedded as BoW (Bag of Words), but performs poorly on other embeddings generated from RoBERTa. GraphSAGE, in contrast, performs poorly on BoW but shows a good performance otherwise. Thus which embeddings are used when comparing models has a large effect on which model appears to be the better model. We see the same effect in \Cref{tab:instruments}. Comparing the two tables we see that in the case of the RoBERTa Encoded and RoBERTa embeddings the order of the models changes, this likely comes from the training effects described in \citet{shchur2018pitfalls}.

\Cref{tab:amazon} also signifies the importance of good embeddings as in this case BoW is better than RoBERTa. The complexity of the embeddings does not necessarily improve the efficiency of the classification. This ties into the results of \citet{nt2019revisiting} as the BoW is more informative of the classification containing the label words in the BoW vector. What is also important to note is that when looking at the performance of the GNN against the unconnected model ($\Delta \uparrow$) we see consistency in the difference across the RoBERTa encodings. \emph{This suggests that the ``quality", denoted by how well the simple MLP performs, is a strong indicator of how well a model will perform, rather than the model architecture itself.}

We see an overall decrease in accuracy in \Cref{tab:instruments} across the models but this attributed to the fact that there are more classes for the dataset. We also see that for RoBERTa embeddings the MLP performs poorly though it does occasionally improve on the simpler models, primarily GCN. With more resources it would be better suited to fine-tune RoBERTa (or some other language transformer) to our dataset and use this model as our unconnected model.

\input{tables/electronics}
\input{tables/instruments}

\textbf{Vision Tasks}
\Cref{tab:flickr} demonstrates the same pattern, that the embedding function (in this case a pre-trained vision model) influences which GNN performs the best. It is interesting to note that we see that none of the GAT models achieve the highest accuracy on any of the Flickr\_v2 embeddings. Instead, similar to the RoBERTa embeddings, we see that GraphSAGE performs the best.

It is important to note for VGG16 that the surprisingly poor performance of GNNs is more likely due to the large vector size of more than 25K. With a smaller embedding space better results on par with ResNet may be achieved. Of course, there is also the possibility that the embeddings provided by VGG16 are inferior to ResNet. 

\input{tables/flickr}

\Cref{tab:instruments,tab:amazon}, compared to \Cref{tab:flickr}, have far larger increases in accuracy from the best performing GNN compared to the unconnected models. This is mainly due to the fact that we were unable to fully fine-tune RoBERTa to our datasets given limited hardware and time. We hypothesise that the improvements seen in \Cref{tab:amazon} would be smaller when compared to a fine-tuned RoBERTa. Similarly, we did not attempt to create a GraNet model using VGG16 as the results on Flickr\_v2 are worse than the ResNet models and therefore for Flickr\_v2 a GraNet ResNet is ideal.

\Cref{tab:instruments,tab:amazon}, specifically with BoW, are the only instances where GAT and GAT2 are the best models. Furthermore, the entries for BoW follow results from past papers, in contrast to the results shown on all other embeddings. With the prevalence of BoW as shown in \Cref{tab:dataset-overview} it begs the question as to whether we are optimising for BoW extraction rather than graph information extraction.

% \subsubsection{Observations}

From these results in both language and vision tasks, we make the following key observations:
\begin{itemize}[noitemsep,nolistsep]
    \item The function $f_e$ used to extract \emph{embeddings influences the performance of different GNNs}, so the embeddings should influence the choice of GNNs regardless of the underlying data. 
    \item GNN models do not always outperform simple unconnected models, \emph{graph structure is not enough} to compete against good classifiers.
    \item The choice of an \emph{embedding function contributes more to the final performance} compared to the choice of a GNN model.
\end{itemize}

% \subsection{Testing GraNet}
\subsection{GraNet}

\Cref{tab:granet} demonstrates that extending our standard models with graph connections provides a significant improvement. We see that these GraNet models beat the best performing GNN. The table includes two forms of GraNet models, the fine-tuned models and the trained models.

\textbf{Fine-tuned}
% \label{sec:eval:finetune}
% \lab
In Flickr\_v2, both GraNet and Unconnected Model use either ResNet18 or ResNet50 weights pre-trained on ImageNet \citep{deng2009imagenet} and then fine-tuned on the target dataset. We observe a significant increase ($+1.5 \%, +1.8 \%$) from the GraNet style of training compared to both unconnected models, and improvement ($1.1 \%, 1.7 \%$) on the best performing GNN model. 

Intuitively, GraNet layers reframe graph representation learning from training a GNN on a fixed pre-extracted embedding to training both the GNN and the embedding function ($f_e$) together on the underlying data. There are obviously trade-offs between time and versatility as rather than just training a GNN the embedding function must be trained as well. 
But the current approach of GNN training on images requires human, or other annotators, which is a hidden time cost. By combining the embedding function and GNN we provide a more general model that does not need external annotators and thus can work on any raw images.

\textbf{Trained from Scratch}
% \label{sec:eval:scratch}
In the Amazon datasets we do not have any pre-trained and train the GraNet model from initialised weights rather than fine-tuning. However, we still observe an improvement on both the unconnected model and best performing GNN. The improvement is smaller than in Flickr\_v2 ($+0.1 \%, +0.3 \%$ compared to $1.1 \%, 1.7 \%$). But the training time is quicker ($\sim1$hr compared to $\sim10$hrs for 300 epochs).

In this case we do not have a general model as we rely on BoW embeddings for the GraNet model as well. But we can see that improvements are possible on existing GNN techniques on the embeddings themselves, without having to use large pre-trained models.

\input{tables/granet}

% \subsubsection{Observations}

We also make the following key observations:

\begin{itemize}[noitemsep,nolistsep]
    \item Graph-connecting a pre-trained network \emph{improves performance by fine-tuning feature extraction based on the graph structure}.
    \item GraNet models \emph{outperform their counterparts by facilitating fine-tuning} on the graph dataset.
\end{itemize}

The architecture for each GraNet is a mixture of the best performing GNN for that embedding and the embedding extraction model ($f_e$) (a Multi-Layer Perceptron in the case of Bag of Words). 
%The details of the GraNet models are described in \Cref{sec:app:setup}.

==> old-sections/granet.tex <==
\section{GraNet}
\label{sec:app:setup}

Below are the specifics of the GraNet models we present in this paper

% \subsubsection{GraNet18 and GraNet50}

%To test this theory we graphly-connect ResNet18 and ResNet50 to create GraNet18 and GraNet50 respectively. We use pre-trained ResNet models %citation needed and where they were trained and only change the final fully-connected layer. This allows us to fine tune the models rather than train them from scratch.

%The specific version of $\phi$, $\psi$ and $\gamma$ we use are those described in GATv2 in \Cref{eq:GATv2}. We alter this method of attention to fit \Cref{eq:transferlearning2} by replacing the input to $\phi$, $\bm{\Theta}\bm{h}_i$, with $f^l_{\bm{\theta}_l}\left( \bm{h}_i \right)$ where $f^l$ is a single layer in ResNet.

%Combining \Cref{eq:GATv2} and \Cref{eq:transferlearning2} we arrive at the following equation 

%\begin{equation}
%    \label{eq:GraNet}
%    \alpha_{ij} = \frac{exp(\bm{a}^T\mbox{LeakyReLU}([f^l_{\bm{\theta}_l}\left( \bm{h}_i \right)||f^l_{\bm{\theta}_l}\left( \bm{h}_j \right)]))}{\sum_{k \in \mathcal{N}_i} exp(\bm{a}^T\mbox{LeakyReLU}([f^l_{\bm{\theta}_l}\left( \bm{h}_i \right)||f^l_{\bm{\theta}_l}\left( \bm{h}_j \right)]))}
%\end{equation}

%This allows us to freeze the weights of the ResNet model and only train the attention mechanism $\bm{a}$. As this is equivalent to training GATv2 we use the same sampler, GraphSAINTRandomWalkSampler, and learning rate. We do however reduce the number of samples as GATv2 ordinarily uses 6000 roots which is too large of a batch size for ResNet.

%Due to hardware limitations we are only able to graphly-connect a subset of layers within ResNet and we present the results detailing which layers we connected.

\subsection{Flickr\_v2 GraNet}

Graphly connecting every layer in a large pre-trained model is hardware intensive. Therefore, rather than graph-connect every single layer in a pre-trained network $f_{\bm{\theta}}$ we can graph-connect only the final layer. We thus split the model into two portions: the first set of unconnected layers and the final GraNet layer.

We can therefore look at equation \Cref{eq:granet} and see in this case that we partially carry out the forward pass of $f_{\bm{\theta}}$ which we will denote as $f_e$ and then carry out a forward pass through a GraNet layer. This allows us to ignore all the steps involved in applying $f_e$ and focus on the final GraNet layer. Denoting this final GraNet as $g$ we achieve the following equation

\begin{equation}
    y = g(f_e(\bm{X}))
\end{equation} 

where y is our output for the given task.

$f_e(\bm{X})$ is the same as described in \Cref{sec:related} and indeed if we were to freeze $f_{\bm{\theta}}$ this would be equivalent to training GraNet with a single layer on the embeddings created by embedding function $f_e$. So instead we also allow $f_e$ to train thus fine-tuning the weights $\bm{\theta}$ of $f_{\bm{\theta}}$. This indirectly allows $f_{\bm{\theta}}$ to learn the graph structure by providing $g$ with better embeddings.

\subsection{Amazon GraNet}

In the case of the Amazon dataset we found that bag of words embedding performed the best. As this does not have an associated pre-trained model we design a multi-layer perceptron (MLP) as a baseline. We then convert all the layers within the MLP to GraNet layers. 

However, a single layer of an MLP is $f^l_{\bm{\theta}_l} \left( \bm{x} \right) = \bm{\theta}_l \bm{x}$. This would therefore mean that \Cref{eq:granet} becomes

\[
\alpha_{ij} = \frac{exp(\bm{a}^T\mbox{LeakyReLU}([\bm{\theta}_l\bm{h}_i||\bm{\theta}_l\bm{h}_j]))}{\sum_{k \in \mathcal{N}_i} exp(\bm{a}^T\mbox{LeakyReLU}([\bm{\theta}_l\bm{h}_i||\bm{\theta}_l\bm{h}_j]))}
\]

This is incredibly similar to \Cref{eq:GATv2,eq:GAT} with the only difference being when we apply the weight matrix, concatenation and attention mechanism. We find this model behaves the same as GAT2 and therefore, given the small size tried a different approach as a comparison.

We introduce a new weight matrix $\mathbf{A}$, to replace $\bm{a}$, as our attention matrix. This allows more complex interactions between the node representations to be exploited by our attention. As demonstrated in \Cref{tab:flickr} in \Cref{sec:app:results} we do see an increase in accuracy.

This approach was too costly to apply to a pre-trained CNN as the size of $\mathbf{A}$ far too large.

==> old-sections/hyperparameters.tex <==
\section{Hyperparameters}
\label{sec:app:hyperparameters}

\Cref{tab:hyperparameters} details the layers of each model used providing the output hidden features of each layer, the sampler used (the specifics shown in \Cref{tab:samplers}) and the maximum and minimum learning rates. Where there is a difference in learning rates we use a learning rate scheduler that decreases the learning rate when validation accuracy plateaus. Where two models use the same sampler the parameters of those samplers are identical to keep consistency across the tests.

In the case of GraNet we start with a high learning rate for 20 epochs with the pre-trained model frozen to allow the GNN to train. We then unfreeze the entire model dropping the learning rate sharply and train for another 100 epochs. In the first stage no learning rate scheduler is employed, same as for all GNNs, and in the second stage we apply the learning rate scheduler.

For GraphSAINTSampler all setups use a walk length of 2 with 5 steps sampling 100 nodes per node for normalisation calculation.

\input{tables/hyperparameters}
\input{tables/sampler-setup}

==> old-sections/introduction.tex <==
%\vspace{-15pt}
\section{Introduction}

Graph Neural Networks (GNNs) have been successful on a wide array of applications ranging from computational biology \citep{zitnik2017predicting} to social networks \citep{Hamilton:2017tp}. The input for GNNs, although sourced from many different domains, is often data that has been preprocessed to a computationally digestible format.
%, normally, in a continuous{\color{blue} is that a factually correct statement? } vector space
These digestible formats are commonly known as embeddings.

Currently, improvements made to GNN architecture are tested against these embeddings and the state of the art is determined based on those results. However, this does not necessarily correlate with the GNNs accuracy on the underlying dataset and ignores the influence that the source and style of these embeddings have on the performance of particular GNN architectures. To test existing GNN architectures, and demonstrate the importance of the embeddings used in training them, we provide three new datasets each with a set of embeddings generated using different methods.
% In this way we analyse 

We further analyse the benefit of using GNNs on fixed embeddings. We compare GNNs to standard models that have been trained or fine-tuned on the target raw data; these models treat each data point as unconnected, ignoring the underlying graph information in data. This simple unconnected baseline surprisingly outperforms some strong GNN models. This then prompts the question: \emph{Will mixing the two approaches unlock the classification power of existing unconnected models by allowing them to utilize the graph structure in our data?} 

Based on the question above, we propose a new method of mixing GNNs with unconnected models, allowing them to train simultaneously. To achieve this we introduce a variation of the standard message passing framework. With this new framework a subset of the unconnected model's layers can each be graph-connected -- exploiting useful graph structure information during the forward pass. We demonstrate that this new approach improves the accuracy of using only a pre-trained or fine-tuned  model and outperforms a stand-alone GNN on a fixed embedding.

We call this new approach \textbf{GraNet} (\underline{Gra}ph-connected \underline{Net}work), and in summary, this paper has the following contributions:

\begin{itemize}[noitemsep]
    \item We provide new datasets and a rich set of accompanying embeddings to better test the performance of GNNs.
    \item We empirically demonstrate that only some existing GNNs improve on unconnected model accuracy and those that do vary depending on the embeddings used. We urge that unconnected models be used as a baseline for assessing GNN performance.
    \item We provide a new method, named GraNet, that combines GNNs and  models (fine-tuned or trained from scratch) to efficiently exploit the graph structure in raw data.
    \item We empirically show that GraNet outperforms both unconnected models (the strong baseline) and GNNs on a range of datasets and accompanying embeddings.
\end{itemize}
%\vspace{-10pt}

==> old-sections/methodology.tex <==
\section{Method}
\label{sec:method}

Our proposed method of converting standard neural network models into graph-connected models blends the two networks. This approach can easily be broken down into individual layers. Taking $f^l_{\bm{\theta}_l}$ as the $l$-th layer in a standard model, $f_{\bm{\theta}}$, where we may be given pre-trained weights $\bm{\theta}$ we can describe this new layer by reformulating \Cref{eq:messagepassing} as such

%\begin{equation}
%\label{eq:transferlearning}
%\mathbf{h}_i^{l} = \gamma_{\bm{\theta}_\gamma} \left(\mathbf{h}^{l-1}_i,
%        \psi_{j \in \mathcal{N}(i)} \left( \phi_{\bm{\theta}_\phi}
%        \left(\mathbf{h}^{l-1}_i, \mathbf{h}^{l-1}_j,\mathbf{e}_{j,i},f_{\bm{\theta}_{l-1}}^{l-1}\right) \right) \right)
%\end{equation}

%A more standard reformulation would be

\begin{equation}
\label{eq:granet}
\vh_i^{l} = \gamma_{\vtheta_\gamma} \left(\vh^{l-1}_i,
        \psi_{j \in \sN(i)} \left( \phi_{\vtheta_\phi}
        \left(f^{l-1}_{\vtheta_{l-1}} \left( \vh^{l-1}_i \right), f^{l-1}_{\vtheta_{l-1}} \left( \vh^{l-1}_j \right), \ve_{j,i}\right) \right) \right)
\end{equation}
%\vspace{-10pt}

where $\mathbf{h}^0_i = \mathbf{x}_i$ rather than applying an embedding function.

% This reformulation highlights how we apply the subsequent layers of the pre-trained model $\mathcal{F}_e$ to each node representation to generate a new representation.

\begin{figure}[ht]
  %\vspace{-10pt}
  \caption{Graphical representation of how our proposed GraNet layer operates for image networks}
  \centering
  \includegraphics[scale=0.35]{figures/ColorBlind.drawio.pdf}
  \label{fig:GraNet}
  %\vspace{-10pt}
\end{figure}

\Cref{fig:GraNet} is a representation of \Cref{eq:granet} specifically in the case where the pre-trained model is a CNN and
($f^{l-1}_{\bm{\theta}_{l-1}}$) is a convolutional layer. The light blue regions perform the standard convolution feature extraction, these extracted feature maps are then adjusted, in the light orange region, by a Message Passing layer with graph attentions. These two representations are then combined.

The light blue regions and resulting channel stacks,
%for a single batch (batch size is $1$)
$A_i \in \sR^{1 \times C_l \times H_l \times W_l}$ through $A_n \in \sR^{1 \times C_l \times H_l \times W_l}$, represent the forward pass through a single CNN layer $f^{l-1}_{\vtheta_{l-1}}$. $A_i$ represents the forward pass of the current node $\vh_i$ and $A_{\{j, \dots, n\}}$ represent the forward pass of the neighbours of $\vh_i$. 
The light orange region and resulting channel stacks, $\mathcal{B}$, represent the graph-based Message Passing stage where the new representations are altered ($\phi_{\vtheta_\phi}$), aggregated ($\psi$) and finally combined with the current node representation ($\gamma_{\vtheta_\gamma}$), following the description in \Cref{eq:granet}.
%\vspace{-10pt}

% Below are the specifics of the GraNet models we present in this paper.

\subsection{GraNet for Flickr\_v2}
\label{sec:method:flickr}

Interconnecting every layer in a large pre-trained model is computationally intensive. Therefore, rather than interconnect every single layer in a pre-trained network $f_{\vtheta}$ we can graph-connect only the final layer. We thus split the model into two portions: the first set of unconnected layers and the final GraNet layer.

We can therefore look at equation \Cref{eq:granet} and see in this case that we partially carry out the forward pass of $f_{\vtheta}$ which we will denote as $f_e$ and then carry out a forward pass through a GraNet layer. This allows us to ignore all the steps involved in applying $f_e$ and focus on the final GraNet layer. Denoting this final GraNet as $g$, and output classification $y$, we achieve the following equation

\begin{equation}
    y = g(f_e(\mX))
\end{equation} 

$f_e(\mX)$ is the same as described in \Cref{sec:related} and indeed if we were to freeze $f_{\vtheta}$ this would be equivalent to training GraNet with a single layer on the embeddings created by embedding function $f_e$. So instead we also allow $f_e$ to train thus fine-tuning the weights $\vtheta$ of $f_{\vtheta}$. This indirectly allows $f_{\vtheta}$ to learn the graph structure by providing $g$ with better embeddings. 
% Intuitively, this not only allow the classifier $g$ to learn from an embedding, but also optimizes the embedding function $f_e$ to help $g$'s learning. 

As GraphSAGE performed the best on ResNet embeddings we use this as our GNN, $g$. As $f_{\vtheta_f}$ is already pre-trained but $g_{\vtheta_g}$ is not fine-tuning the model produces poor results. We therefore initially train $g_{\vtheta_g}$ on a frozen ${f_e}_{\vtheta_f}$, after this short training period we unfreeze ${f_e}_{\vtheta_f}$ allowing both to train fine-tuning the weights $\vtheta_g$ and $\vtheta_f$.

\subsection{GraNet for Amazon}
\label{sec:method:amazon}

In the case of the Amazon dataset we found that Bag of Words embedding performed the best. As this does not have an associated pre-trained model we design a multi-layer perceptron (MLP) to compare against. We then convert all the layers within the MLP to GraNet layers. \emph{This method is therefore not fine-tuned but trained from initialised weights.}  

We also find that GAT \citep{Brody2021GATv2,Velickovic:2018we} models perform the best on this task. We therefore use graph attention message passing as shown in \Cref{eq:GATv2} for our GraNet model. Keeping in line with \Cref{eq:granet} the new graph attention mechanism becomes

\begin{equation}
    \alpha_{ij} = \frac{exp(\bm{a}^T\mbox{LeakyReLU}([f^l_{\vtheta_l}(\bm{h}_i)||f^l_{\vtheta_l}(\bm{h}_j)]))}{\sum_{k \in \sN_i} exp(\bm{a}^T\mbox{LeakyReLU}([f^l_{\vtheta_l}(\bm{h}_i)||f^l_{\vtheta_l}(\bm{h}_j)]))}
\end{equation}

However, a single layer of an MLP is $f^l_{\vtheta_l} \left( \vx \right) = \vtheta_l \vx$. This would therefore mean that \Cref{eq:Gatv3} becomes

\begin{equation}
    \label{eq:Gatv3}
    \alpha_{ij} = \frac{exp(\va^T\mbox{LeakyReLU}([\vtheta_l\vh_i||\vtheta_l\vh_j]))}{\sum_{k \in \sN_i} exp(\va^T\mbox{LeakyReLU}([\vtheta_l\vh_i||\vtheta_l\vh_j]))}
\end{equation}

This is very similar to \Cref{eq:GATv2} with the only difference being when we apply the weight matrix, concatenation and attention mechanism. We find this model behaves the same as GAT2 and therefore, given the small size tried a different approach as a comparison.

Rather than use the vector parameter $\va$ we introduce a linear function $a_{\vtheta_a}: \sR^{2F} \rightarrow \sR^{F^\prime}$ that takes the LeakyReLU of the concatenation of a node, $f_{\vtheta_l}(\vh_i)$, and its neighbour, $f_{\vtheta_l}(\vh_i)$, as input. The result is a feature vector in a new feature space, though in our case we have $F^\prime = F$. This allows more complex interactions between the node representations to be exploited by our attention. This approach is too costly to apply to a pre-trained CNN as the size of $\bm{\theta_a}$ is far too large.

==> old-sections/related-datasets.tex <==
\section{An In-depth Overview of Existing Datasets}
\label{sec:app:dataset-overview}

Due to the discussed importance of $f_e$ on GNN performance there is a lot to discuss about prior datasets that exist within the space of GNNs in regards to these functions.

% \subsubsection{Torchvision}

% \textbf{UNCERTAIN WHAT TO DISCUSS HERE}

% Though this paper focuses on graphly-connected datasets there is still a discussion to be had about existing datasets outside of graphly-connected ones. It can be argued that these datasets employ some embedding function $f_e$ as the images provided in these datasets need to be scaled and normalised. But these transformations are not embedding functions which is an important distinction.

\subsection{Pytorch Geometric}
\label{sec:app:pyg}

Pytorch Geometric python library provides a standard interface on top of Pytorch to allow for the development of graph based machine learning. The library also provides a sample of datasets from previous papers published in this field. A brief overview of popular graph-connected datasets, their task and embeddings is available in table \ref{tab:dataset-overview}.

As is clear from the table the current standard embedding for datasets is bag of words. In the cases where bag of words approaches are not used the approach is grounded in classical text representations such as n-grams and word vectors.

The tasks in these popular datasets are node classification where the node data is frequently text. We therefore say that on the node level these are text classification tasks. The only instance of a non-text classification task is Flickr \cite{zeng2019graphsaint}, though based on the fact that the underlying data is image descriptions this could also be considered a text classification task.

This demonstrates how limited the reach of GNNs currently stand as they are being trained on datasets that behave very similarly where the only difference is the specifics of the available data. We feel that this does not therefore fully test the capabilities of GNNs and puts too much emphasis on bag of words and text classification.

\subsection{Open Graph Benchmark}

The results in this paper focus on \textit{node property prediction} as the data that unconnected models ordinarily work on is easily transferred to nodes in a graph. So when discussing Open Graph Benchmark  \citep[OGB]{hu2020open} the focus is on the node property prediction subset (OGBN). 

The goal of OGB is to create a standard set of datasets that can be used to compare different GNN architectures so a discussion as to way we did not use their datasets is warranted. The available datasets \textit{ogbn-products, ogbn-proteins, ogbn-arxiv, ogbn-papers100M} and \textit{ogbn-mag} all use variations on the same text representations used in \Cref{sec:app:pyg}. These include Bag of Words (BoW), word2vec and skip-gram. This means the same discussions on these classical text holds here. 

We see that the majority of the tasks focus on text classification, excluding \textit{ogbn-protein}, this again draws into question how well these datasets are testing the range of classification tasks. Further to this, focusing mainly on BoW style embeddings raises the question of whether we are building good BoW extractors or graph information extractors.

We do not compare against these datasets as information on how they extracted and washed their data is not readily available and therefore finding matching raw data was not possible. Without the matching raw data we cannot compare a raw version of the dataset to the embedding dataset provided by OGBN.

\subsection{Flickr}
The prior Flickr dataset used in \textit{Zeng et al.} \cite{zeng2019graphsaint} originated from \textit{McAuley et al.} \cite{McAuley2012image} which aimed to utilize network connections and image descriptions rather than the images themselves. The specific embedding function that the paper used is Bag of Words.
% , where the input dataset $\bm{X}$ is the descriptors of and image and the embedding function $f_e$ is function that takes a descriptor and returns a vector representing which of the top 500 words of the entire dataset $\bm{X}$ were present.

This embedding function is a valid representation of images but it is not easily applicable to other image datasets. Thus GNNs trained on this dataset are confined to images with descriptions that have been transformed using the same top 500 words. Noting that this list of top 500 words is not readily available.

\subsection{Amazon}
\textit{Zeng et al.} \cite{zeng2019graphsaint} also provide an Amazon dataset (AmazonProducts) covering the entirety of Amazon. Without a known source we instead use available Amazon databases online to download and generate our own dataset. The embedding function  used is to tokenise the reviews by 4-grams and take the single value decomposition. This is, as with Flickr, not easily applicable outside of the original dataset.

An alternative Amazon dataset (Amazon) is also available from \textit{Shchur et al.} \cite{shchur2018pitfalls} created originally in \textit{McAuley et al.} \cite{McAuley2016image}. Though the original source of the dataset used a pre-trained Caffe model to embed the product images this dataset did not use these. Instead they created their own embeddings using the bag of words standard with the product reviews as the raw data.

==> old-sections/related.tex <==
\section{Related Work}
\label{sec:related}

\textbf{Graph Augmented Networks} \citet{chen2021on} introduce Graph-augmented MultiLayer Perceptrons (GA-MLPs) as a simplified alternative to Graph Neural Netwroks (GNNs). These models involve a two step process - augmenting the node features of the graph based on the topology and then using these node features applying a learnable function at the node level. This allows a fixed graph operator and two sets of MultiLayer Perceptrons (MLPs) be used to extract features from the graph. This approach is related to similar simplified GNN techniques \citep{wu2019simplifying,nt2019revisiting}. The paper proves that this simplified approach is not as expressive as standard GNNs when looking at the Weisfeiler-Lehman test for distinguishing non-isomorphic graphs. This suggests that GNNs are well suited for inferring information based on graph structure but the paper does not comment on which approach is best in practice. We differ in our approach to augmenting networks with graph structure by using existing GNNs and do not attempt to simplify the network. We do provide a graph-connected MLP but this looks at adding message passing to MLPs rather than separte funcitons on the graph data.
 
\textbf{Effect of training on GNN performance} \citet{shchur2018pitfalls} look at the effect of hyperparameters and training in GNNs to show that these have dramatic effect on model ordering. Simply changing the split on a dataset caused large changes in accuracy and which GNN performed best, even though the hyperparameters of the GNNs remained constant. We show similar large difference when considering different embeddings with the same splits across embeddings. 

\textbf{Ablation studies on GNNs} Further to these discoveries \citet{nt2019revisiting} demonstrate that GNNs only utilise the graph structure to de-noise already highly informative features. They go as far as to demonstrate in certain conditions GNNs and MLPs perform the same. \citet{chen2019powerful} demonstrate that linearising the graph filter stage of GNNs does not hinder but actually increases the performance. Similarly \citet{wu2019simplifying} simplify GNNs by removing non-linearity between layers allow for pre-computing the $k$ message passes. This reduces graph representation learning to a simple linear regression. In all of these cases they demonstrate that the major contribution of GNNs is in their graph structure capabilites. We do not analyse these aspects but look at how this capability can be used in existing unconnected networks.

==> old-sections/reproducibility.tex <==
\section{Reproducibility}

We discuss how we setup all of our experiments in \Cref{sec:setup} including how many runs we completed for each data-point. the specific random seeds that we used for the three runs were 42, 9001 and 27032002. The number of runs for each run is also listed here and for the models that have a different number of epochs the specifics are mentioned in \Cref{sec:app:hyperparameters}.

All test runs were carried out on a single Nvidia A100 80GB GPU, we used pytorch 1.12 with cuda 11.3. All other packages where installed based on these requirements.

\Cref{sec:app:hyperparameters} also contains the specific architectures, samplers, learning rates and learning rate schedulers used in each of the model test runs. These are also linked back to \citet{zeng2019graphsaint} to provide comparable results to the ones achieved in that paper for similar datasets Flickr and Amazon.

\Cref{sec:app:datasets} details the specifics of how we formed our datasets including how we downloaded the raw data, steps we took to wash the data, how we formed the graph and how we created our embeddings. The specifics of how we labelled the data and the labels that we chose are also available.

We have anonymised the dataset including the specific code used to create GraNet models, the config files used and the code to download, wash and build the datasets available \href{https://anonymous.4open.science/r/Revisiting-Embeddings-for-Graph-Neural-Networks}{here}.



==> old-sections/results.tex <==
\section{Detailed Results}
\label{sec:app:results}

% \Cref{tab:flickr,tab:instruments} both demonstrate similar results to those seen in \Cref{tab:amazon}. 

% \Cref{tab:flickr} demonstrates the same pattern, that the embedding function (in this case a pre-trained vision model) influences which GNN performs the best. We do not provide a BoW embedding for Flickr\_v2 as there is no text for raw images. It is interesting to note that we see that none of the GAT models achieve the highest accuracy on any of the Flickr\_v2 embeddings. Instead, similar to the roBERTa embeddings, we see that GraphSAGE performs the best. This is the reason we chose GraphSAGE for our Flickr\_v2 GraNet models.

% It is important to note for VGG16 that the surprisingly poor performance of GNNs is more likely due to the size of the embedding produced by VGG16, 25088. With a smaller embedding space, potentially by using layers within the VGG16 classifier, may produce better results on par with ResNet. But there is also the possibility that, similar to roBERTa, VGG16 provides worse embeddings than ResNet. Further tests were not carried on VGG16 due to limitations with time.

% In comparison to \Cref{tab:amazon} we see a far smaller increase in accuracy from the best performing GNN compared to the unconnected pre-trained model. This is mainly due to the fact that we were unable to fully fine-tune roBERTa to our datasets given limited hardware and time and hypothesise that the improvements seen in \Cref{tab:amazon} would be smaller when compared to a fine-tuned roBERTa. Similarly, we did not attempt to create a GraNet model using VGG16 as, for one, the results on Flickr\_v2 are worse than the ResNet models but also due to a limitation of resources.

% \Cref{tab:instruments} demonstrates very similar results to \Cref{tab:amazon} which is to be expected as they are generated in the same way. We see an overall decrease in accuracy across the models but this attributed to the fact that there are more classes for the dataset. 

\Cref{tab:amazon-std,tab:instruments-std,tab:flickr-std,tab:granet-std} are the same results as those present in \Cref{sec:eval} but with added standard deviation from the mean.

\input{tables/flickr-std}
\input{tables/instruments-std}
\input{tables/electronics-std}
\input{tables/granet-std}

==> old-sections/setup.tex <==
\section{Experimental Setup}
\label{sec:setup}

For all test results we run 3 train-test runs each with a different random seed and take the arithmetic mean and include the standard deviation. The three random seeds are the same for every entry in the table for fair comparison. The architecture used for each benchmark GNN is identical across all datasets and embeddings. Training takes 300 epochs of training unless otherwise stated.

Where a Graph Neural Network (GNN) is used as part of a GraNet model (as described in \Cref{sec:method}) the same sampler is used for consistency. The specific architectures used are designed using the hyperparameters in \citet{zeng2019graphsaint}. In the case of GraphSAGE the learning rate was decreased to improve convergence. For specific details of each architecture and learning rate see \Cref{sec:app:hyperparameters}.

\subsection{Datasets}

An overview of the datasets is provided below with the specific metrics for each dataset shown in \Cref{tab:flickr-dataset}. A more detailed discussion is available in \Cref{sec:app:datasets}. \emph{It is important to note that though these datasets mirror prior datasets due to the need for raw data we diverge from these datasets}. Therefore we do not make any direct comparisons to previous datasets though the results we achieve on our new datasets are on par with results seen in prior papers.

\subsubsection{Flickr\_v2}
\label{sec:setup:flickr}

The underlying data $\bm{X}$ is raw images and so Convolutional Neural Networks (CNNs) are used as embedding functions. As a sample of existing pre-trained CNNs we use ResNet18, ResNet50 \citep{he2016deep} and VGG16 \citep{simonyan2015very}. In all three cases we use the pre-trained models provided by TorchVision, using the feature vectors after the final pooling stage before the classification stage. 

It is important to note that \emph{there is no Bag of Words (BoW) embedding for Flickr\_v2 because there is no sensible object that can be considered a ``word" for raw image data.} The available Flickr \citep{zeng2019graphsaint} uses BoW because the underlying data is image text descriptions not raw images. This limits how a GNN, or general neural network, can classify images as the images must first be processed to provide text descriptions. 
%This would either require a human, and thus the major benefit of using a neural network (time efficiency of classification) is lost, or another neural network which our approach generalises to. Therefore, only raw images or pre-trained CNN embedding functions are used.

\subsubsection{AmazonElectronics and AmazonInstruments}

The underlying data $\bm{X}$ is text so text classification transformers such as RoBERTa \citep{liu2019roberta}
are ideal, specifically we use pre-trained RoBERTa.
We extract three different embeddings from RoBERTa using the pre-trained model provided by fairseq toolkit \citep{ott2019fairseq}. The first is the byte pair tokenisation used by RoBERTa, the second is the feature extraction provided by fairseq which occurs after RoBERTa's transformer heads and before classification, and the final is the feature vector present before the last fully connected layer. Due to restrictions in the token size for RoBERTa we remove all nodes that have reviews with greater than 512 tokens.

We also provide the standard Bag of Words embedding as in the case of text classification this is a common embedding practice, keeping in line with prior datasets \citep{Kipf:2017tc,zeng2019graphsaint}
we use the top 500 words to create our Bag of Word embeddings.

==> tables/dataset-electronics.tex <==
\begin{table}[!h]
	\centering
	\caption{AmazonElectronics}
	\label{tab:amazon-dataset}
	\begin{tabular}{ccccc}
		\toprule
		\multicolumn{1}{c}{Embedding} &
		\multicolumn{1}{c}{Number of Nodes} &
		\multicolumn{1}{c}{Number of Classes} &
		\multicolumn{1}{c}{Input Shape}\\
		\midrule
		Bag of Words & 92048 & 6 & (500) \\
		roBERTa Byte Pair & 92048 & 6 & (512) \\
		roBERTa Encoded & 92048 & 6 & (1024) \\
		roBERTa & 92048 & 6 & (1024) \\
		\bottomrule
	\end{tabular}
\end{table}

==> tables/dataset-flickr.tex <==
\begin{table}[!ht]
	\centering
	\caption{The number of nodes and classes with the shape of the data $x_i$ for the three new datasets with each of the different embedding functions used. Note that Flickr\_v2 also has the raw images represented by -}
	\label{tab:flickr-dataset}
	\begin{tabular}{ccccc}
		\toprule
		\multicolumn{1}{c}{Dataset} &
		\multicolumn{1}{c}{Embedding} &
		\multicolumn{1}{c}{\# Nodes} &
		\multicolumn{1}{c}{\# Classes} &
		\multicolumn{1}{c}{Input Shape}\\
		\midrule
		\multirow{4}{*}{Flickr\_v2}
		& - & 76659 & 7 & (3, 224, 224) \\
		& ResNet50 & 76659 & 7 & (1024) \\
		& ResNet18 & 76659 & 7 & (512) \\
		& VGG16 & 76659 & 7 & (25088) \\
		\midrule
		\multirow{4}{*}{AmazonElectronics}
		& Bag of Words & 92048 & 6 & (500) \\
		& RoBERTa Byte Pair & 92048 & 6 & (512) \\
		& RoBERTa Encoded & 92048 & 6 & (1024) \\
		& RoBERTa & 92048 & 6 & (1024) \\
		\midrule
		\multirow{4}{*}{AmazonInstruments}
		& Bag of Words & 21127 & 7 & (500) \\
		& RoBERTa Byte Pair & 21127 & 7 & (512) \\
		& RoBERTa Encoded & 21127 & 7 & (1024) \\
		& RoBERTa & 21127 & 7 & (1024) \\
		\bottomrule
	\end{tabular}
\end{table}

==> tables/dataset-instruments.tex <==
\begin{table}[!h]
	\centering
	\caption{AmazonInstruments}
	\label{tab:instrument-dataset}
	\begin{tabular}{ccccc}
		\toprule
		\multicolumn{1}{c}{Embedding} &
		\multicolumn{1}{c}{Number of Nodes} &
		\multicolumn{1}{c}{Number of Classes} &
		\multicolumn{1}{c}{Input Shape}\\
		\midrule
		Bag of Words & 21127 & 7 & (500) \\
		roBERTa Byte Pair & 21127 & 7 & (512) \\
		roBERTa Encoded & 21127 & 7 & (1024) \\
		roBERTa & 21127 & 7 & (1024) \\
		\bottomrule
	\end{tabular}
\end{table}

==> tables/dataset-overview.tex <==
\begin{table}[!ht]
    %\vspace{-10pt}
	\centering
	\caption{An overview of popular datasets}
	\label{tab:dataset-overview}
	\adjustbox{scale=.82}{
	\begin{tabular}{ccccc}
		\toprule
		\multicolumn{1}{c}{Name} &
		\multicolumn{1}{c}{Info Source} &
		\multicolumn{1}{c}{Classes} &
		\multicolumn{1}{c}{Feature Length} &
		\multicolumn{1}{c}{Embedding} \\
		\midrule
		Amazon \citep{shchur2018pitfalls} 
		& Text & 10, 8 & 767, 745 & Bag of Words \\
		AmazonProducts \citep{zeng2019graphsaint} & Text & 107 & 200 & 4-gram with SVD \\
		Flickr \citep{zeng2019graphsaint} & Image & 7 & 500 & Bag of Words \\
		Reddit \citep{zeng2019graphsaint,Hamilton:2017tp} & Text & 41 & 602 & Avg. GloVe vectors \\
		Cora \citep{Kipf:2017tc} & Text & 7 & 1,433 & Bag of Words \\
		CiteSeer \citep{Kipf:2017tc} & Text & 6 & 3,703 & Bag of Words \\
		PubMed \citep{Kipf:2017tc} & Text & 3 & 500 & Bag of Words \\
		\bottomrule
	\end{tabular}
	}
	%\vspace{-10pt}
\end{table}

==> tables/electronics-gc.tex <==
\begin{table}[!h]
	\centering
	\caption{Comparison of graphly-connected MLP to the best performing GNN on AmazonElectronics}
	\label{tab:amazon-gc}
	\begin{tabular}{cc}
		\toprule
		\multicolumn{1}{c}{Model} & 
		\multicolumn{1}{c}{Bag of Words} \\
		\midrule
		GAT2 & \textit{81.8} \\
		MLP Baseline & 71.6 \\
		\midrule
		GraNet & \textbf{81.9} \\
		\bottomrule
	\end{tabular}
\end{table}

==> tables/electronics.tex <==
\begin{table}[!ht]
\vspace{-10pt}
	\centering
	\caption{Test accuracy on AmazonElectronics with different embeddings compared against a standard unconnected MLP model. The embedding styles are explained in \Cref{sec:app:datasets}, \Cref{tab:flickr-dataset}.}
	\label{tab:amazon}
	\adjustbox{max width=\textwidth}{
	\begin{tabular}{ccccc}
		\toprule
		\multirow{2.5}{*}{Model} & 
		\multicolumn{4}{c}{Embedding styles} \\
		\cmidrule(lr){2-5} &
		\multicolumn{1}{c}{Bag of Words} & 
		\multicolumn{1}{c}{Byte Pair} &
		\multicolumn{1}{c}{RoBERTa Encoded} & 
		\multicolumn{1}{c}{RoBERTa}\\
		\midrule
		Unconnected MLP & 71.6\% (+0.0) & 21.6\% (+0.0) & 55.8\% (+0.0) & 51.9\% (+0.0) \\
		\midrule
		GCN & 69.1\% (-2.5) & 21.7\% (+0.1) & 22.7\% (-33.1) & 22.3\% (-29.6) \\
		GAT & \textit{81.1\% (+10.5)} & 22.2\% (+0.6) & 46.1\% (-9.7) & 40.3\% (-11.6) \\
		GAT2 & \textbf{81.8\% (+10.2)} & 22.2\% (+0.6) & 41.8\% (-14.0) & 35.7\% (-16.2) \\
		GraphSAGE (Random) & 71.3\% (-0.3) & \textit{26.8\% (+5.2)} & \textit{57.0\% (+1.2)} & \textit{53.7\% (+1.8)} \\
		GraphSAGE (Neighbour) & 76.4\% (+4.8) & \textbf{40.4\% (+20.8)} & \textbf{67.8\% (+12.0)} & \textbf{66.4\% (+12.5)} \\
		\bottomrule
	\end{tabular}
	}
%\vspace{-10pt}
\end{table}

==> tables/flickr.tex <==
\begin{table}[!ht]
	\centering
	\caption{Test accuracy on Flickr\_v2 with different embeddings, compared against the corresponding unconnected vision model. Included is the difference $\Delta$ of each model to the unconnected model and the standard deviation of each result. The details of the embedding styles are available in \Cref{sec:app:datasets}.}
	\label{tab:flickr}
	\begin{tabular}{cccc}
		\toprule
		\multirow{2.5}{*}{Model} & 
		\multicolumn{3}{c}{Embedding Styles} \\
		\cmidrule(lr){2-4} &
		\multicolumn{1}{c}{ResNet18} & 
		\multicolumn{1}{c}{ResNet50} &
		\multicolumn{1}{c}{VGG16} \\
		\midrule
		%Unconnected Model & 45.2\% (+0.0) & \textit{46.9\% (+0.0)} & \textbf{47.0 (+0.0)} \\
		%\midrule
		GCN & 41.8\% (-3.4) & 38.3\% (-8.6) & \textbf{35.5\% (-11.5)} \\
		GAT & 38.1\% (-7.1) & 37.1\% (-9.8) & 27.3\% (-19.7) \\
		GAT2 & 42.1\% (-3.1) & 41.0\% (-5.9) & 34.2\% (-12.8) \\
		GraphSAGE (Random) & \textit{45.4\% (+0.2)} & \textbf{47.0\% (+0.1)} & \textit{35.2\% (-11.8)} \\
		GraphSAGE (Neighbour) & 
		\textbf{45.8\% (0.6)} & 44.5\% (-2.4) & 34.5\% (-12.5) \\
		\bottomrule
	\end{tabular}
\end{table}

==> tables/granet-std.tex <==
\begin{table}[!ht]
	\centering
	\caption{Comparison of GraNet models against the best performing GNNs for a specific embedding. Included is the difference $\Delta$ of each model to the unconnected model and the standard deviation of each result. The specifics of the 3 datasets is explained in \Cref{sec:app:datasets}.}
	\label{tab:granet-std}
	\begin{tabular}{ccccc}
		\toprule
		\multirow{2.5}{*}{Model} & 
		\multicolumn{2}{c}{Flickr\_v2} & 
		\multicolumn{1}{c}{Electronics} & 
		\multicolumn{1}{c}{Instruments} \\
		\cmidrule(lr){2-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} &
		\multicolumn{1}{c}{ResNet18} & 
		\multicolumn{1}{c}{ResNet50} & 
		\multicolumn{1}{c}{Bag of Words} & 
		\multicolumn{1}{c}{Bag of Words} \\
		\midrule
		Unconnected Model & 45.2\% $\pm$ 0.1 & 46.9\% $\pm$ 0.0 & 71.6\% $\pm$ 0.3 & 66.1\% $\pm$ 0.2 \\
		$\Delta \uparrow$ & +0.0 & +0.0 & +0.0 & +0.0 \\
		\midrule
		GAT2 & 42.1\% $\pm$ 1.8 & 41.0\% $\pm$ 1.5 & \textit{81.8\%} & \textit{79.4\% $\pm$ 0.3} \\
		$\Delta \uparrow$ & -3.1 & -5.9 & \textit{+10.2} & \textit{+13.3} \\
		
		GraphSAGE (Random) & 45.4\% $\pm$ 0.1 & \textit{47.0\% $\pm$ 0.0} & 71.3\% & 67.5\% $\pm$ 0.3 \\
		$\Delta \uparrow$ & +0.2 & \textit{+0.1} & -0.3 & +1.4 \\
		
		GraphSAGE (Neighbour) & 
		\textit{45.8\% $\pm$ 0.2} & 44.5\% $\pm$ 0.1 & 76.4\% & 72.6\% $\pm$ 0.3 \\
		$\Delta \uparrow$ & \textit{+0.4} & -2.4 & +4.8 & +6.5 \\
		
		\midrule
		% GraNet (incorrect attention) & (45.2)  & (46.9) \\
		GraNet & 
		\textbf{46.7\% $\pm$ 0.1} & \textbf{48.7\% $\pm$ 0.1} & \textbf{81.9\% $\pm$ 0.5} & \textbf{79.7\% $\pm$ 0.9} \\
		$\Delta \uparrow$ & \textbf{+1.5} & \textbf{+1.8} & \textbf{+10.3} & \textbf{+13.6} \\
		\bottomrule
	\end{tabular}
\end{table}

==> tables/granet.tex <==
\begin{table}[!h]
    % \vspace{-10pt}
	\centering
	\caption{Comparison of GraNet models against the best performing GNNs for a specific embedding. Unconnected Model refers to ResNet18 or ResNet50, in the case of Flickr\_v2, and an MLP otherwise. The setup of each GraNet model is detailed in \Cref{sec:method:flickr,sec:method:amazon} and the specifics of the 3 datasets can be found in \Cref{sec:app:datasets}.}
	\label{tab:granet}
	\adjustbox{max width=\textwidth}{
	\begin{tabular}{ccccc}
		\toprule
		\multirow{2.5}{*}{Model} & 
		\multicolumn{2}{c}{Flickr\_v2} & 
		\multicolumn{1}{c}{Electronics} & 
		\multicolumn{1}{c}{Instruments} \\
		\cmidrule(lr){2-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} &
		\multicolumn{1}{c}{ResNet18} & 
		\multicolumn{1}{c}{ResNet50} & 
		\multicolumn{1}{c}{Bag of Words} & 
		\multicolumn{1}{c}{Bag of Words} \\
		\midrule
		Unconnected Model & 45.2\% (+0.0) & 46.9\% (+0.0) & 71.6\% (+0.0) & 66.4\% (+0.0) \\
		\midrule
		GAT2 & 42.1\% (-3.1) & 41.0\% (-5.9) & 
		\textit{81.8\% (+10.2)} & 
		\textit{79.4\% (+13.0)} \\
		
		GraphSAGE (Random) & 45.4\% (+0.2) & 
		\textit{47.0\% (+0.1)}& 
		71.3\% (-0.3) & 67.5\% (+1.1) \\
		
		GraphSAGE (Neighbour) & 
		\textit{45.8\% (+0.4)} & 
		44.5\% (-2.4) & 
		76.4\% (+4.8) & 
		72.6\% (+6.2) \\
		
		\midrule
		% GraNet (incorrect attention) & (45.2)  & (46.9) \\
		GraNet & 
		\textbf{46.7\% (+1.5)} & 
		\textbf{48.7\% (+1.8)} & 
		\textbf{81.9\% (+10.3)} & 
		\textbf{79.7\% (+13.3)} \\
		\bottomrule
	\end{tabular}
	}
%\vspace{-20pt}
\end{table}

==> tables/instruments.tex <==
\begin{table}[!ht]
	\centering
	\caption{Test accuracy on AmazonInstruments with different embeddings compared against a standard unconnected MLP model. Included is the difference $\Delta$ of each model to the unconnected MLP and the standard deviation of each result. The embedding styles are explained in \Cref{sec:app:datasets}.}
	\label{tab:instruments}
	\adjustbox{max width=\textwidth}{
	\begin{tabular}{ccccc}
		\toprule
		\multirow{2.5}{*}{Model} & 
		\multicolumn{4}{c}{Embedding Styles} \\
		\cmidrule(lr){2-5} &
		\multicolumn{1}{c}{Bag of Words} & 
		\multicolumn{1}{c}{Byte Pair} &
		\multicolumn{1}{c}{RoBERTa Encoded} & 
		\multicolumn{1}{c}{RoBERTa} \\
		\midrule
		Unconnected MLP & 66.1\% (+0.0) & 21.0\% (+0.0) & 43.9\% (+0.0) & 39.8\% (+0.0) \\
		\midrule
		GCN & 64.0\% (-2.1) & 20.8\% (-0.2) & 20.4\% (-23.5) & 20.4\% (-19.4) \\
		GAT & \textit{79.3\% (+13.2)} & 21.6\% (+0.6) & 47.5\% (+3.6) & 46.1\% (+6.3) \\
		GAT2 & \textbf{79.4\% (+13.3)} & 21.2\% (+0.2) & \textit{49.8\% (+5.9)} & \textit{47.8\% (+8.0)} \\
		GraphSAGE (Random) & 67.5 (+1.4)\% & \textit{23.9\% (+2.9)} & 45.1\% (+1.2) & 41.9\% (+2.1) \\
		GraphSAGE (Neighbour) & 72.6\% (+6.5) & \textbf{43.4\% (+22.8)} & \textbf{62.4\% (+18.5)} & \textbf{59.9\% (+20.1)} \\
		\bottomrule
	\end{tabular}
	}
\end{table}
